(De-)Randomized Smoothing for Decision Stump Ensembles

Tree-based models are used in many high-stakes application domains such as finance and medicine, where robustness and interpretability are of utmost importance. Yet, methods for improving and certifying their robustness are severely under-explored, in contrast to those focusing on neural networks. Targeting this important challenge, we propose deterministic smoothing for decision stump ensembles. Whereas most prior work on randomized smoothing focuses on evaluating arbitrary base models approximately under input randomization, the key insight of our work is that decision stump ensembles enable exact yet efficient evaluation via dynamic programming. Importantly, we obtain deterministic robustness certificates, even jointly over numerical and categorical features, a setting ubiquitous in the real world. Further, we derive an MLE-optimal training method for smoothed decision stumps under randomization and propose two boosting approaches to improve their provable robustness. An extensive experimental evaluation on computer vision and tabular data tasks shows that our approach yields significantly higher certified accuracies than the state-of-the-art for tree-based models. We release all code and trained models at https://github.com/eth-sri/drs.

==> methods_verifier.tex <==

\subsection{Convex Relaxation of NODE Layers} \label{sec:trafo-node}
While the discrete step sizes introduced with our controlled adaptive ODE solver ensures that there is only a finite number of trajectories our solver can take for any input region, naively computing bounds for all of them independently would still be intractable. 

To tackle this problem, we construct a graph representation of the ODE solve for an input set, which we call the trajectory graph $\bc{G}(\Gamma({\mathcal{Y}}))= (\bc{V}, \bc{E})$, where the nodes $v \in \bc{V}$ correspond to solver states, over-approximated using the \boxd domain and identified by the tuple $(t, h)$ of time and step size, and the directed edges $e \in \bc{E}$ are part of trajectories the solver might have taken. This allows us to merge solver states that share time and step size, vastly reducing the number of trajectories we have to consider (quadratic in the integration time instead of exponential).


\paragraph{Verification with Box}
Given an input \boxd $\hat{\vx}_{0,0}$, we construct our trajectory graph as follows:
We use standard propagation with the box domain to compute an interval over-approximation of the local error estimate $\hat{\delta}_{(t, h)}$ at every solver step and check which time step updates (increase, decrease, or accept) could be made according to \cref{eq:modified-update}. For each possible update, we thus obtain a new state tuple $(t_\text{new}, h_\text{new})$ with corresponding box approximation of the state and add the node $(t_\text{new}, h_\text{new})$ with an edge from $(t, h)$ to $(t_\text{new}, h_\text{new})$ to the graph. If the node $(t_\text{new}, h_\text{new})$ already existed, we update its state to contain the convex hull of the two box approximations. If multiple updates are possible, we call this trajectory splitting. We repeat this process, processing nodes in order of increasing time $t$ and decreasing time step $h$. We thus have to traverse every node at most once, until only the node $(T_\text{end}, 0)$ has not been processed at which point we have completed the graph generation. We thus obtain a box over-approximation of the solver state $\vy_{L}$ at $T_\text{end}$ and thus the output of the NODE layer, which we can now propagate through the rest of the network for verification or provable training.

We illustrate this construction process in \cref{fig:trajectory-graph}, where we highlight newly added edges and nodes in red and the processed node in blue: We initialize the graph with the node $(0, h_0)$, where in our case $h_0 = 1/2$ (see \cref{fig:trajectory-graph}(a)). We now do an abstract solver step for this node and find that $\delta > \tau_\alpha$. Thus, we either accept the step, yielding the next node $(1/2, 1/2)$, or we reject the step and decrease the time step by $\alpha=2$, yielding the node $(0, 1/4)$, both connected to the current node (see \cref{eq:modified-update} (b)). We now choose among the nodes without outgoing edges the one with the smallest current time and largest time step, $(0,1/4)$ in our case, and do another abstract solver step, yielding $\delta < 1$. We thus either accept the step, yielding the node $(1/4,1/4)$, or additionally increase the time step, yielding the node $(1/4,1/2)$ (see \cref{eq:modified-update} (b)). We proceed this way until the only node without outgoing edges is the termination node $(T_\text{end},0)$, where $T_\text{end} = 0$ in our case.

\begin{figure*}
    \centering
    \include{figures/graph} %
    \caption{ An example construction trajectory graph $\mathcal{G}(\Gamma({\mathcal{Y}}))$ for a controlled adaptive ODE solver with $h_0 = \frac{1}{2}$, $\alpha = 2$ and $T_{end} = 1$. Trajectory splitting occurs in all vertices except the final state, whereas trajectory merging occurs in all vertices except the initial state.} \label{fig:trajectory-graph}
\end{figure*}


\paragraph{Verification with \deeppoly}
When verifying with the \deeppoly domain, we have already computed linear constraints with respect to the  output state $y_{(T_{end}, \ 0)}$ of the node (as discussed in \cref{sec:background}), and wish to propagate them backward through the node to obtain constraints with respect to the input state $y_{(0, \ h_0)}$.
We first construct the complete trajectory graph, either using \boxd as described above or using \deeppoly, following the same approach as described below.
During this process, we retain concrete element-wise upper- and lower-bounds.

We now back-propagate our relational constraints through the graph as follows:
We select an arbitrary node with no outgoing edges, back-substitute the constraints with respect to the corresponding solver state along all incoming edges (corresponding to solver steps), and remove that node as well as all traversed edges from the graph. We repeat this step until the only remaining node is the input node $(0, h_0)$, giving us one set of constraints, that we can back-substitute through the rest of the network, allowing verification with \deeppoly

The core challenge is that for states where the trajectory split, i.e., nodes with more than one outgoing edge, we obtain several sets of linear constraints. We thus have to merge these constraints in a sound manner without losing too much precision. We call this the linear constraint aggregation problem (\lcap).

\paragraph{Linear Constraint Aggregation Problem}\label{sec:DPCA}
Here, we solve the problem of soundly merging a set of different linear constraints bounding the same output depending on which trajectory was taken to compute it.
Let us consider $m$ different linear upper-bounds $r^+_i(\vx) = \va^+_i \vx + c^+_i$ on $y$ with respect to $\vx$ as defined in \cref{eq:deeppoly} and inducing the constraining set $\{[\vx, r^+_i(\vx)] \subseteq \R^{d+1} \mid \vx \in \bc{B} \}_{i=1}^m$, where $\vx$ is bounded by the hyper-box $\bc{B} := [\vl, \vu] \subseteq \R^d$.
We now want to compute the linear constraint $\hat{r}^+(\vx) = \hat{\va}^+_i \vx + \hat{c}$ minimizing the volume below the constraint over $\vx \in \bc{B}$, while soundly over, approximating all other constraints.
More formally, we want to solve:
\begin{align}\label{eq:lcap}
(\hat{\va}^+, \hat{c}) =& \argmin_{[\va^+, c] \in \R^{d+1}} \int_{\bc{B}} \va^+ \vx + c \mathrm{d}\vx \label{eq:LCAP} \\
	s.t. \quad & \va^+ \vx + c \geq \max_i \va^+_i \vx + c_i, \quad \forall \vx \in \bc{B}\\
		      =& \argmin_{[\va^+, c] \in \R^{d+1}} \va^+ \frac{\vl + \vu}{2} + c  \label{eq:dpcap2}\\ 
	s.t. \quad & \va^+ \vx + c \geq \max_i \va^+_i \vx + c_i, \quad \forall \vx \in V(\bc{B})
\end{align}
where $V(\bc{B})$ are the $2^d$ corners of the hyper-box $\bc{B}$ and showing soundness on $V(\bc{B})$ is sufficient due to the linearity of all constraints. While we can thus encode the \lcap as an LP, we have to consider exponentially many soundness constraints (one per corner), making the exact solution intractable. We thus propose the \rm, which we will explain next.

\paragraph{\rm}
The \rm over-approximates the optimal solution of the \lcap by first translating the $\max$ operator into a composition of ReLU functions
and then applying the \deeppoly ReLU transformer.
More concretely, let us denote the maximal value of $r^+_i$ as $\overline{r}^+_i = \max_{\vx \in \bc{B}} r^+_i(\vx)$ and assume w.l.o.g. $\overline{r^+_{1}} \geq \dots \geq \overline{r^+_m}$. We now iteratively combine two constraints $r^+_1$ and $ r^+_2$ into one upper bounding constraint $r^+_{1,2} \geq \max(r^+_1, r^+_2)=  r^+_1 + \text{ReLU}(r^+_2 - r^+_1)$ to obtain 
\begin{align*}
\max_{j\in [m]}r^+_j & = \max(r^+_m, \dotsc, r^+_3, \max(r^+_2,r^+_1))\\ 
&\leq \max(r^+_m, \dotsc, r^+_3, r^+_{1,2}) \leq \max(r^+_m, \dotsc,, \max(r^+_3, r^+_{1,2}))\\ &\leq \dots \leq \hat{r}^+.
\end{align*}
We visualize this for a $1$-d problem in \cref{fig:aggregation}, where the first iteration already yields the constraint $r^+_{1,2} = \hat{r}^+$, dominating the remaining $r^+_3$.

\begin{figure}
	\centering
	\mysubfigure[0.24\textwidth]{
		\centering
		\includegraphics[width = \textwidth]{figures/dpcap_1.pdf}  
	}{DPCAP with $m=3$ and $d=1$. \label{fig:DPAC}}
	\mysubfigure[0.24\textwidth]{
		\centering
		\includegraphics[width=1\textwidth]{figures/dpcap_2.pdf}  
	}{First iteration of ReLU-method.\label{fig:relu-iter-1}}
	\mysubfigure[0.24\textwidth]{
		\centering
		\includegraphics[width=1\textwidth]{figures/dpcap_3.pdf}  
	}{Final output of the ReLU-method. \label{fig:relu-iter-2}}
	\mysubfigure[0.24\textwidth]{
		\centering
		\includegraphics[width=1\textwidth]{figures/legend_dpcap.pdf}  
	}{Legend. \label{fig:legend-DPCAP}}
	\caption{Visualization of the DPCAP with $m=3$ and $d=1$. Additionally, we show the output of the ReLU-method after one iteration (b) and the final output (c).}
	\label{fig:aggregation}
\end{figure}


\subsection{Provable Training}
Considering the full trajectory graph is infeasible for training, even when only using the \boxd domain. However, it is also not necessary to consider every trajectory to obtain an optimizable approximation of the worst case loss. 
We thus compute a \boxd approximation of the \node layer by considering only up to $\kappa$ selected trajectories $\mathcal{S}(\Gamma({\mathcal{Y}}))$ without any merging.

We select trajectories as follows: We first compute the reference trajectory $\Gamma(y^*)$, where $y^*$ corresponds to the unperturbed input and propagate a \boxd abstraction of the NODE input through the NODE layer, until we reach the termination time $T_\text{end}$. If multiple time step updates are possible, i.e., we encounter trajectory splitting, we choose a single path via random sampling, and add the corresponding state to the branching point set $\mathcal{C}$. We now repeat this process with an intermediate state sampled from the set of branching points, until we have considered $\kappa$ trajectories. Finally, we compute the \boxd output of the NODE layer as the over-approximation of all obtained final states. During sampling of initial states and the branching decisions, we balance exploration of the full trajectory graph and staying close to the reference trajectory. For more details, please see \cref{app:node_trafo_details}.

\paragraph{Loss Functions} For provable training we use a loss term of the following loss form:
\begin{align} \label{eq:cert-loss}
\bc{L}(\vx,y) &= (1 - \sfrac{\epsilon'}{\epsilon}) \bc{L}_\text{std}(\vx,y) + \sfrac{\epsilon'}{\epsilon} \bc{L}_\text{rob}(\vx,y) + \omega \|\vu_\text{out}-\vl_\text{out}\|_1,
\end{align}
where $\bc{L}_\text{std}$ is the loss evaluated on the unperturbed sample, $\bc{L}_\text{rob}$ is an over-approximation of the worst case loss computed by propagation the input region $\bc{B}^{\epsilon'}$ through the network, and $\vu_\text{out}-\vl_\text{out}$ the width of the corresponding output region.
During training, we use $\epsilon$ annealing, gradually increasing $\epsilon'$ from $0$ to $\epsilon$, thereby shifting focus from the standard to the robust loss term. In the classification setting, we use the cross entropy loss and in time series forecasting we use a latent ODE specific loss, combining a MAE error and ELBO term, defined in \cref{eq:forecasting-loss-background}.

\paragraph{Stabilizing Training}
In the time-series forecasting setting, the long integration times involving many solver calls lead to very large effective model depths. There $\epsilon$-annealing alone is insufficient to stabilize the training in the face of an exponential accumulation of approximation errors.
To combat this, we additionally anneal the abstract ratio $\rho$ from $0$ to $1$ and only use non-zero perturbation magnitudes for the last $\rho L$ data points in every time series, i.e., for an input with time index $j$, we set$\epsilon' \gets \epsilon' \mathds{1}_{j < \rho L} $. We visualize this annealing process in \cref{fig:annealing} and highlight, that it is independent of $\epsilon$-annealing.

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{figures/eps_annealing.png}
		\vspace{-5mm}
		\caption{Only $\epsilon$ annealing.}
		\label{fig:eps-annealing}
	\end{subfigure}
	\begin{subfigure}[b]{0.8\textwidth}
		\includegraphics[width=\textwidth]{figures/eps_rho_annealing.png}
		\vspace{-5mm}
		\caption{Annealing $\epsilon$ and abstract ratio $\rho$.}
		\label{fig:rho-annealing}
	\end{subfigure}
	\vspace{-2mm}
	\caption{Comparison of time-series input with just $\epsilon$-annealing (top) or additionally $\rho$-annealing (bottom) where dots indicate concrete inputs and error bars abstract regions.}
	\label{fig:annealing}
\end{figure}

